Combined Acoustic and Pronunciation Modelling for Non-Native Speech Recognition

In this paper, we present several adaptation methods for non-native speech recognition. We have tested pronunciation modelling, MLLR and MAP non-native pronunciation adaptation and HMM models retraining on the HIWIRE foreign accented English speech database. The ``phonetic confusion'' scheme we have developed consists in associating to each spoken phone several sequences of confused phones. In our experiments, we have used different combinations of acoustic models representing the canonical and the foreign pronunciations: spoken and native models, models adapted to the non-native accent with MAP and MLLR. The joint use of pronunciation modelling and acoustic adaptation led to further improvements in recognition accuracy. The best combination of the above mentioned techniques resulted in a relative word error reduction ranging from 46% to 71%.

==> ttt <==
This paper presents a fully automated approach for the recognition of non-native speech based
on acoustic model modification. For a native language (L1) and a spoken language (L2), pronunciation
variants of the phones of L2 are automatically extracted from an existing non-native database
as a confusion matrix with sequences of phones of L1. This is done using L1's and L2's ASR systems. This confusion concept deals with the problem of
non existence of match between some L2 and L1 phones.
The confusion matrix is then used to modify the acoustic models (HMMs) of L2 phones by integrating corresponding L1 phone models as alternative
HMM paths. In this way, no lexicon modification is carried.
The modified ASR system achieved an improvement between 32\% and 40\% (relative, L1=French and L2=English) in WER on the French non-native database used for testing.
